Connectivity in mobile device-to-device networks in urban environments

In this article we setup a dynamic device-to-device communication system where devices, given as a Poisson point process, move in an environment, given by a street system of random planar-tessellation type, via a random-waypoint model. Every device independently picks a target location on the street system using a general waypoint kernel, and travels to the target along the shortest path on the streets with an individual velocity. Then, any pair of devices becomes connected whenever they are on the same street in sufficiently close proximity, for a sufficiently long time. After presenting some general properties of the multi-parameter system, we focus on an analysis of the clustering behavior of the random connectivity graph. In our main results we isolate regimes for the almost-sure absence of percolation if, for example, the device intensity is too small, or the connectivity time is too large. On the other hand, we exhibit parameter regimes of sufficiently large intensities of devices, under favorable choices of the other parameters, such that percolation is possible with positive probability. Most interestingly, we also show an in-and-out of percolation as the velocity increases. The rigorous analysis of the system mainly rests on comparison arguments with simplified models via spatial coarse graining and thinning approaches. Here we also make contact to geostatistical percolation models with infinite-range dependencies.

==> Sec_Simulator.tex <==
In this section we describe algorithms and ideas for the {\em Python} simulator that we used to create the illustrations in the current report and which will be used for the simulation results, such as for example the propagation speed of the malware or the percolation behavior of the model, presented in Report 3. 

Compared to the simulators developed by the Orange teams, the main selling point of our simulation ansatz is the continuous-time modeling approach. To be more precise, when implementing an agent-based model, the default approach is usually to iterate the model in small, discrete time steps of size $\eps>0$. The new position and state of the agents at time $t + \eps$ is determined from the state of the agents at time $t$. 
Currently two ongoing internships at Orange develop simulators in discrete time to understand percolation behavior and infection spreading in a system of agents that includes mobility based on street systems. The main benefit of this discrete-time ansatz lies in both, its intuitive implementation and its fast run-time, at least if a multi thread approach is used.
The main drawback of the discrete-time approach however lies in the accumulated inaccuracies stemming from the discrete step size as well as the fact that relevant characteristics of the model can only be evaluated at the discrete time steps. 
We believe that these inaccuracies become especially important if multiple layers of randomness are involved. In particular, we here recall that the movement of the agents influences the spread of the malware in the system. In order to reduce this accumulated inaccuracies, it is necessary to reduce the step-size of the model, which leads to  slower run-times. 

Already in an earlier collaboration between Orange and WIAS~\cite{CRE3} a simulation ansatz has been initially developed that is based on an event queue that runs in continuous time.
Now, in this current project, we further develop and generalize this ansatz. 

The main idea behind an {\em event queue} is the removal of fixed time steps in favor of agent-based time steps. Any agent is only updated if a relevant event occurs in the system. Relevant events for agents include the arrival on a new street, reaching its destination, getting infected, or getting cured.

In the following, similar to Section~\ref{sec_model}, we give a detailed description of our simulator by considering first the street system, then the devices and their paths through the street system, and finally how we build connections between devices. 

\subsection{Street systems on a torus}
The goal of the simulations is to understand the characteristics (connectedness, speed of propagation,\dots) of the process defined on $\R^2$, and compute them. 
However, simulation are only possible on bounded areas. In particular, in order to approximate the characteristics of the unbounded area from bounded areas, we have to deal with boundary effects and small-volume errors. 
Let us mention that in previous joint projects (see for example \cite{CRE2} and \cite{CRE3}) it turned out to be sufficient to simulate a larger area for the street system and then use a smaller area in the interior as an observation window.
Although we could in principle replicate this ansatz here, the added movement of the devices holds a challenging problem: As the movement of devices is the limiting factor in the simulation time, we do not want to simulate devices outside the simulation area. 

One solution to get a realistic movement scheme, is to generate a street system on a torus. To our knowledge there exists no pre-defined python library to generate a Poisson--Voronoi tessellation on a torus. However, we were able to use the \emph{scipy.spacial} library that generates a planar Poisson--Voronoi tessellation, by using eight identical copies (organized as non-overlapping cells surrounding the central original cell) of the points generating the tessellation. 
% (see Figure\red{TODO}).
From this augmented tessellation we are able to derive our street system on the torus, which we describe next. 

We use the {\em NetworkX python package} as a graph structure for both, the street system as well as the connectivity graph formed by the devices on the streets. Although both generation time and storage space of this structure are slightly larger than pure lists of coordinates and an adjacency matrix, we believe that the already implemented and optimized utilities more than compensate for this. The structure allows easy storage of marks associated to both, edges and vertices, in order to store important quantities like positions, lengths of streets, devices on streets and many more. Furthermore, we are able to use the provided shortest-path and clustering algorithms directly implemented in $C$. Whenever we refer to saved information of a street $s$ or a device $X$ we will put the saved attribute as an index, e.g., $s_{\rm length}$, which is chosen in order to facilitate a comparison to the Python code. 

In order to derive the torus structure from the eight identical copies of the points generating the tessellation, we iterate over all the associated edges. If both endpoints lie inside the central original cell we can import the edge directly. If exactly one edge lies inside the original cell, the edge goes through the torus boundary. Hence, we now have to find the matching edge on the other side of the torus. We obtain the position of the corresponding edge by mapping the corner that lies outside the torus to its corresponding point inside the torus. To be more precise, we denote by $L$ the side length of the central cell and define the mapping $m \colon (x,y)\in L^2 \mapsto [-L,L]^2$ as 
\begin{align}\label{eq-projection-torus}
m(x,y) = \big(((x + L) \mod 2L) - L, ((y + L) \mod 2L) - L\big).
\end{align}
Note that the most efficient way to obtain the point from its position would be another sorting of all the corners and a bin-search with a smaller radius, as the exact position of the matching point is known.
% For simplicity (and as the generation of the street system is not the bottleneck in the code) saved the edge and do the matching lat

Once we have identified the corresponding point on the torus, we connect the endpoints of the torus. However, we set the \emph{length} of the connection to the length of the original street and not the euclidean distance between the points, as the shortest connection goes through the torus boundary. With the help of {\em Thales's intercept theorem} we are able to calculate and save the exact point where the direct edge goes through the boundary of the torus and re-emerges on the opposite side. This information is only used for display purposes and can be omitted when doing the simulations.

In order to prepare for the following initialization of the devices, and in particular the generation of a destination via a probability kernel, we discretize the torus into squares of small side length and associate to each square the Voronoi cells that intersect the square. 


\subsection{Initialization of initial device positions, destinations and shortest paths}
After generating the street system, on each street $s$ on the torus we generate the initial device positions with linear intensity with respect to the length of the street $s$. Recall that the number of devices on each street is given by $\text{Poi}(\la s_{\rm length})$, where $\text{Poi}(\cdot)$ is a random variable with Poisson distribution. Then, for each individual initial device position, we can determine its location on the street using a $\text{uniform}([0,1])$ variable $p$. In general, positions of devices are not saved in terms of absolute coordinates $(x,y)$. Instead, we save them as a linear combination of the two endpoints of the street it is currently located on $(v^{(1)}, v^{(2)},p)$. 
Let us mention that $(v^{(1)}, v^{(2)},p)$ and $(v^{(2)}, v^{(1)},1-p)$ refer to the same point. We will always save the position of a device in such a way that the positional argument increases as the device moves, in other words, that the devices moves in the direction from the first vertex to the second and save the tuple in $X_{\rm pos}$.

For $X_{\rm pos} = (v^{(1)}, v^{(2)},p)$ let us denote by $a(X_{\rm pos})= (1-p){v^{(1)}}_{\rm pos} + p{v^{(2)}}_{\rm pos}$ the coordinates of the position on the torus. When the value of an attribute is a tuple, we use the following notation to isolate certain elements of the tuple, $X_{\rm pos}=(X_{\rm pos}[0],X_{\rm pos}[1], X_{\rm pos}[2]).$ Let us mention that one benefit of using linear combinations lies in the fact that for the movement and the calculation of the contact times of the devices, the absolute coordinates are not required: Two devices $X^{(1)}$ and $X^{(2)}$ on the same street are in contact if $|X^{(1)}_{\rm pos}[2]-X^{(2)}_{\rm pos}[2]|\cdot s_{\rm length} \le r$. The same holds for the position of the device after any  updating. When we update the position $p$ of a device $X$ to a fixed time $t_{\rm new}$, the new position is given by 
$$p_{\rm new} = p_{\rm old} + (t_{\rm new}-X_{\rm time})\cdot X_{\rm velocity}/s_{\rm length},$$
and we have to update the time at which the position of the device was determined, $X_{\rm time} =t_{\rm new}$. Here we denoted the velocity of $X$, independently generated from $\muv$, as  $X_{\rm velocity}$.

In our simulations, we used the kernel $\k'$. We pick a uniform point on a ball around the home with radius $R$ with the help of polar coordinates. More precisely, let $U_1$ and $U_2$ be two independent uniform $[0,1]$ variables. Then
\begin{align*}
D=(x+\sqrt{U_1}R\sin(2\pi U_2), y+\sqrt{U_1}R\cos(2\pi U_2))
\end{align*}
is uniformly distributed in a disk around $(x,y) = a(X_{\rm pos})$ with radius $R$. If $D$ is outside the torus, we map it back inside using the mapping $m$ from \ref{eq-projection-torus}.
Now we have to project $D$ to the closest street. Let us observe, that the closest street to $D$ is part of the boundary of the Voronoi that includes $D$.
We are able to find this Voronoi cell using the discretization of the torus that was produced at the end of the previous subsection. Now, it remains to calculate the projection of $D$ to all the edges of the Voronoi cell. Finally, a comparison of the distance of all edges towards $D$ yields $D'= q(D)$. 
%. The position of $D'$ is saved as $($

Having done the steps we just described, next, we have to calculate the shortest path between the home of $X$ and its destination $D'$.
Let us assume that $D'$ is not on the same street as $X$ (in this case the shortest path is trivial). Both $X$ and $D'$ lie on a street (an edge of the street graph) and not directly on a crossing (the vertices of the street graph). As shortest path algorithms calculate the shortest path between vertices.
In order to directly use the shortest path algorithms directly, instead of comparing the four shortest path connecting the crossings of the streets $X$ and $D'$ lie on (we don't know which crossing is used to leave/enter the streets), we add both $X$ and $D'$ as temporary points to the street system. For $X$, we add the temporary edges $\overline{Xv^{(1)}}$ of length $ps_{\rm length}$ and $\overline{Xv^{(2)}}$ of length $(1-p)s_{\rm length}$, where $s$ is the street containing $X$. After adding the edges leading to $D$, we apply the shortest-path algorithm of NetworkX to obtain the shortest path and save it in $X_{\rm path}$. If the shortest path from $X$ to $D$ goes through $v^{(2)}$, we have to change $X_{\rm pos}$ to $(v^{(2)}, v^{(1)}, 1-p)$ due to the convention that those linear combinations are always saved such that $p$ increases. As $X$ and $D$ were temporary vertices in the street system, we have to remove them after the calculation of the shortest path finishes.


We finish the initialization of the model by calculating the (future) contacts of the devices. For each pair $X^{(i)}, X^{(j)}$ of devices on the same street $s$ both their relative position on the street and their velocities are known. If the devices move in the same direction, we solve 
$$ | X^{(i)}_{\rm pos}[2] s_{\rm length} + X^{(i)}_{\rm velocity} t - (X^{(j)}_{\rm pos}[2] s_{\rm length} + X^{(j)}_{\rm velocity} t |)$$
in order to compute the interval $[\max(c_{\rm min},0), c_{\rm max}]$ where the devices will be in contact, not regarding the events that a device reaches a corner or its destination (in those cases the contact times have to be re-calculated. We  create an edge $\overline{X^{(i)}, X^{(j)}}$
 and save the contact interval in the attribute $\overline{X^{(i)}, X^{(j)}}_{\rm c-time}$. Let us note that, if $X^{(i)}$ and $X^{(j)}$ have the same velocity and move in the same direction, the devices will either never have contact (we do not generate an edge) or are in contact to each other forever ($\overline{X^{(i)}, X^{(j)}}_{\rm c-time}= [0, \infty]$). 

After initialization, we have two different NetworkX graphs: A graph $G_S$ that represents the street system and a separate Graph $G_{\rm D}$ of devices.
Any vertex $V$ of $G_S$ represents a crossing and has only the attribute $V_{\rm pos}$ as its $x,y$-coordinate. Any edge $s$ in $G_S$  represents a street and carries both $s_{ \rm length}$ and $s_{ \rm devices}$, the length of the street and the set of devices on the street. For display purposes only, we save whether and where the edge goes through the boundary of the torus. On the other hand, a Vertex $X$ of $G_{\rm D}$ has more attributes. We save its last calculated position $X_{\rm pos}$, the time at which $X$ was at that position  $X_{\rm time}$ (as the simulation is run in continuous time and device positions are only updated when necessary), its velocity $X_{\rm velocity}$, and  $X_{\rm path}$ ,the path that the device is going to take. Furthermore, in order to simulate the propagation of malware in Report 2 and Report 3, we track $X_{\rm state}$.
For edges $e$ of $G_{\rm D}$ we track the time two devices will be in contact in $e_{\rm c-time}$ and we track in $e_{\rm connection}$ if a successful connection was established.
    

\subsection{Variable time steps via event queues}
As we mentioned in the introduction of this section, the sampling of the simulation does not happen in fixed time steps. Instead, we use a queue to schedule events that may occur in the format \emph{(time, event type, additional information)}. Then, the event queue is a collection of such tuples that are ordered by their first component in ascending order.

We are going to track the following six event types:
\begin{itemize}
\item[(1)] A device becomes infected
\item[(2)] A device becomes cured
\item[(3)] A device reaches a crossing, i.e., leaves a street and enters a new street
\item[(4)] A device reaches its destination
\item[(5)] Update to a fixed time
\item[(6)] Finish the simulation
\end{itemize}
The main idea behind the performance improvement is that at each event, only the device that caused the event gets updated, the rest of the system stays untouched.
The events described in (1) and (2) are placeholder events that are later needed for the system described in Report 2 in which infected devices and white knights are introduced. Event (5) is only used to evaluate the state of the whole system at a fixed time whereas event (6) is used to finish the simulation at time $T$.

We start by initializing the event queue by generating the first events. Each device generates exactly one event for the event queue.
If the next location that the device will reach on its path is the destination $D= (v_1, v_2, p)$ (both $X$ and $D$ lie on the same street $s=\overline{v_1 v_2}$), we add an event of type (4). 
This happens at time $$t= (p-X_{\rm pos}[2]) \cdot s_{\rm length} /X_{\rm velocity}.$$
Therefore, we add the event $(t, (4), X)$. As additional information we included the name of the device that reaches its destination.


If the next point that the device $X$ reaches along its path to its destination is a crossing, this will happen at time $$t= (1-X_{\rm pos}[2]) \cdot s_{\rm length} /X_{\rm velocity},$$
and we add the event $(t, (3), X)$ to the event queue.
We finish the initialization by adding an event of type (6) at time $T$ to conclude the simulation.

\subsubsection{Event (3): A device reaches a crossing}
Events where devices reach corners are of the form $(t, (3), X)$: Other than the time of reaching the crossing $t$, also the name of the involved device is stored as additional information. 
At time $t$, device $X$ looses contact to all the devices still remaining on the street.
We iterate over the remaining devices on the street to determine if their contact has to be stopped or not. For the additional device $X^{(i)}$ on the same street as $X$, a successful connection is established if 
\begin{align} \label{eq-connectiontime}
\min(\overline{XX^{(i)}}_{c-time}[1],t) - \overline{XX^{(i)}}_{c-time}[0]>\rho.
\end{align}
In this case we set the marker $ \overline{XX^{(i)}}_{\rm connection}$ to \emph{true}.
Afterwards, the edge is deleted, if (either just now, or on a previous street) no connection was established. Let us emphasize that, once a successful connection was established, the edge will not get deleted.
The new street that the device is entering next can be obtained from $X_{\rm path}$. In order to establish the intervals where communication is possible, we update the position of each device from the new street to their position at time $t$. The contact interval can then, like in the initialization of the model, be obtained from the positions and velocities of the devices. At the end of the calculation, both for the time of first contact and the time where the contact is lost, the current time $t$ is added.
 
As a final step we generate the next event for the event queue: If the next point on the path to the destination is another street corner, we add the event
 \begin{align*}
 (t+s_{\rm length}/X_{\rm velocity}, (3), X).
 \end{align*}
 
\subsubsection{Event (4): A device reaches its destination}
Events where devices reach their destination are of the form $(t, (4), X)$. 
Now, the device reverse its traveled path to continue its journey. The old path $X_{\rm path} = [(v_0, v_1,p),v_1,\dots,v_{n-1}, (v_{n-1}, v_n, q)]$  gets updated to 
$$X_{\rm path} = [(v_n, v_{n-1},1-q),v_{n-1},\dots.v_{1}, (v_1,v_0 , 1 - p)].$$
Note that, although $X$ is still in contact with the same devices on its street, the direction of movement on $X$ has changed. For each $X^{(i)}$ on the same street, we check if a connection was already established (see~\ref{eq-connectiontime}). If not, we calculate the new contact time $c_{\rm min}', c_{\rm max}'$. If $c_{\rm min}'< t<c_{\rm max}'$, by a reflection argument also $X_{\rm c-time}[0] <t< X_{\rm c-time}[1]$ and we set $\overline{XX^{(i)}}_{\rm c-time} = [X_{\rm c-time}[0],  c_{\rm max}']$, as the previous time, in which the device was in contact before $t$, has to be kept in mind. Else, there is currently no contact between $X$ and $X_i$ and we set the contact interval to the one we just calculated $\overline{XX^{(i)}}_{\rm c-time}  = [c_{\rm min}', c_{\rm max}']$.

\subsubsection{Events (5), (6) and outlook}
Event (5) is an update to a global time. 
We have to update both the positions of the devices to their new positions and for each edge in $G_{\rm D}$ (that did not previously establish a successful connection), we update its status with the help of~\ref{eq-connectiontime}.

Event (6) is used to stop the simulation at time $T$. In order to generate the final state of the simulation, we replace the whole event queue with a single event of type (5) at time $T$ that updates the system to time $T$. As event (5) does not add additional events, the simulation terminates.

During the work on Report 2, we will implement event (1) and event (2). Here, we are able to build on the code for the propagation of the infection, written for the previous project~\cite{CRE3}, as the implementation of event queues was similar.

%Currently the event-queue holds exactly one event for each device, resulting in a fast run-time.




%\begin{figure}[!htpb]
%\centering
%\input{Picture/pic4_shortest_path.tex}
%\caption{Illustration for }
%\label{Fig_Mobil_2_Points}
%\subsection{The event-queue}
%\end{figure}
